Deep Smartphone Sensors-WiFi Fusion for Indoor Positioning and Tracking

We address the indoor localization problem, where the goal is to predict user's trajectory from the data collected by their smartphone, using inertial sensors such as accelerometer, gyroscope and magnetometer, as well as other environment and network sensors such as barometer and WiFi. Our system implements a deep learning based pedestrian dead reckoning (deep PDR) model that provides a high-rate estimation of the relative position of the user. Using Kalman Filter, we correct the PDR's drift using WiFi that provides a prediction of the user's absolute position each time a WiFi scan is received. Finally, we adjust Kalman Filter results with a map-free projection method that takes into account the physical constraints of the environment (corridors, doors, etc.) and projects the prediction on the possible walkable paths. We test our pipeline on IPIN'19 Indoor Localization challenge dataset and demonstrate that it improves the winner's results by 20\% using the challenge evaluation protocol.

==> macros.tex <==
\usepackage{times,epsfig,graphicx}
\usepackage{algorithm,algorithmic}
\usepackage[usenames]{color}
%\usepackage{amssymb,amsmath}
\usepackage[latin1]{inputenc}
\usepackage{fancyhdr}
\usepackage{verbatim}
\usepackage{tabularx}
%\usepackage{hyperref}
\usepackage{amsthm,amssymb,amsmath}
\usepackage{float}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage{bm}

\newlength{\smallimage}
        \setlength{\smallimage}{0.8cm}
        \setlength\fboxrule{2pt}
        \setlength\fboxsep{0pt}
        \definecolor{rel}{rgb}{.1,.6,.2}
        \definecolor{nrl}{rgb}{1,1,1}
        \definecolor{qim}{rgb}{1,1,1}


%\newcommand{\note}[1]{({\color{green}#1})}
\newcommand{\todo}[1]{({\color{red}ToDo: #1})}
\newcommand{\rk}[1]{{\color{red}{\bf #1}}}
\newcommand{\mk}[1]{{\color{magenta}{\bf #1}}}
\newcommand{\bk}[1]{{\color{blue}{\bf #1}}}
\newcommand{\gk}[1]{{\color{green}#1}}

%\DeclareMathOperator*{\E}{\mathbb{E}} 
\DeclareMathOperator{\E}{\mathbb{E}}

\makeatletter

\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}


\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot} 
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}


%Specific macros for math symbles
\newcommand{\ka}{k\prime}
\newcommand{\ia}{i\prime}
\newcommand{\logl}{\mathcal{L}}
\newcommand{\deriv}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\minus}{\textrm{-}}
\newcommand{\plus}{\textrm{+}}
\newcommand{\Gauss}[3]{\mathcal{N}(#1;#2,#3)}
%\newcommand{\Gaussd}[2]{\mathcal{N}(#2,#3)}
\newcommand{\T}{\top}
\newcommand{\trans}[1]{#1^{\T}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\norm}[1]{\parallel\!#1\!\parallel}
\newcommand{\snorm}[1]{\norm{#1}_2^2}
\newcommand{\snormw}[1]{\norm{#1}_W^2}
\newcommand{\ind}[1]{[\![#1]\!]}
\newcommand{\hinge}[1]{[#1]_{+}}
\newcommand{\dotp}[2]{\langle #1,#2 \rangle}
\newcommand{\bigo}[1]{\mathcal{O}(#1)}
\newcommand{\kl}[2]{\mathcal{D}_{\textsc{KL}}(#1||#2)}
\newcommand{\dwd}{d_{W}^{\textrm{dotp}}}
\newcommand{\rank}[1]{\textrm{rnk}(#1)}

\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\rarr}{$\rightarrow$}
\newcommand{\larr}{$\leftarrow$}
\newcommand{\mysec}[1]{section~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eqp#1{(\ref{eq:#1})}
\def\eq#1{Eq.~\ref{#1}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ben{\begin{eqnarray*}}
\def\een{\end{eqnarray*}}


\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}

\def\algo#1{Algorithm~\ref{algo:#1}}
\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}



\newcommand{\bt}[1]{\begin{tabular}{#1}}
\newcommand{\et}{\end{tabular}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\ul}[1]{\underline{#1}}

%\newcommand{\eq}[1]{(\ref{#1})}

% macros
\def\g{\gamma}
\def\G{\Gamma}
% \def\a{\alpha}
% \def\g{\gamma}
% \def\S{\Sigma}
% \def\s{\sigma}
% \def\o{\omega}
% \def\l{\lambda}
% \def\d{\delta}
\def\N{\mathcal N}
\def\F{\mathcal F}
\def\L{\mathcal L}

\def\diag{\mbox{diag}}

\newcommand{\st}{\textrm{subject to}}
\DeclareMathOperator*{\mini}{minimise}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\trace}{tr}


%% Macros from Jakob Verbeek
\def\code#1{\begin{quote}{\tt #1}\end{quote}}
\def\I{{\rm I\!I}}                            % the indicator function
\def\R{{\rm I\!R}}                            % the real numbers
\def\matlab{\textsc{\small Matlab }}        % matlab add
%\def\Tr#1{\textrm{Tr}\{#1\}}                % trace
\def\diag#1{\textrm{diag}\left( #1 \right)} % diag
\def\Gauss#1#2#3{\mathcal{N}\left(#1 ; #2,#3\right)}   % Gaussian density
\def\ex#1#2{\textrm{I\!E}_{#1}\!\left[#2\right]}     % expectation
\def\half{\frac{1}{2}}              % half
\def\<{\langle}
\def\>{\rangle}

\def\nn{\nonumber}

% BOLD stuff
\def\alphabold{\mbox{\boldmath $\alpha$}}
\def\betabold{\mbox{\boldmath $\beta$}}
\def\gammabold{\mbox{\boldmath $\gamma$}}
\def\mubold{\mbox{\boldmath $\mu$}}
\def\kappabold{\mbox{\boldmath $\kappa$}}
\def\epsbold{\mbox{\boldmath $\epsilon$}}
\def\thetabold{\mbox{\boldmath $\theta$}}
\def\phibold{\mbox{\boldmath $\phi$}}
\def\Upsilonbold{\mbox{\boldmath $\Upsilon$}}
\def\eye{{\bf I}}



%\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45}
%\newcommand{\hide}[1]{}
%\newcommand{\rar}{\rightarrow}
%\newcommand{\lar}{\leftarrow}
%\newcommand{\ol}{\overline}
%\newcommand{\Ra}{\Rightarrow}
%\newcommand{\upA}{\uparrow}
%\newcommand{\si}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bmu}{{\bm \mu}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfA}{{\bf A}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfD}{{\bf D}}

\newcommand{\tbf}{{\tilde{\bf f}}}
%\newcommand{\O}{{\Omega}}
\newcommand{\bfO}{{\bf \Omega}}
\newcommand{\bfG}{{\bf \Gamma}}


\newcommand{\bfh}{{\bf h}}
%\newcommand{\E}{\mathrm{E}}$
\newcommand{\V}{\mathrm{Var}}

\newcommand{\Cov}{\mathrm{Cov}}

%\newcommand{\bfxx}{[\begin{array}{l}{\tilde {\bf x}_n}\\{\tilde {\bf f}({\bf x}_n)\end{array}]}
%\newcommand{\bfwz}{[\begin{array}{l}{\bf w} \\ {\bf z}\end{array}]}

\newcommand{\al}{{\alpha}}
%\DeclareMathOperator*{\E}{\mathbb{E}}

==> soa-activity-detection.tex <==
%-deep learing from smartphone sensor data for activity recognition
\cite{zhou-2019-smartphone}
In the indoor environment, human activity contains rich semantic information, for example, if a user’s activity is recognized as taking an elevator, the location of the user can be inferred to the elevator. These activities can be used as the landmarks for indoor localization and mapping [1–5].
For example, when a user’s activity is detected as “elevator”, his/her location may be at the elevator. The recognition of human activities has been approached in two different ways, namely ambient sensing methods and wearable sensing methods [6]. The ambient sensing methods make use of the devices fixed in predetermined point of interest to sense human activities, such as video camera [7]
and WiFi signal [8]. Wearable sensing methods are based on the sensors attached to the user. Recently, with the development of sensor technology, wearable sensing methods have become more and more popular. The wearable sensing methods can be implemented directly in smartphones [9].

Human activities can be categorized into different types [6], including ambulation (e.g., walking, running, sitting, standing still, lying, climbing stairs, descending stairs, riding escalator, and riding elevator), transportation (e.g., riding a bus, cycling, and driving), daily activities (e.g., eating, drinking,
working at the PC, etc.), exercise/fitness (rowing, lifting weights, spinning, etc.), military (e.g., crawling, kneeling, situation assessment, etc.), and upper body (Chewing, speaking, swallowing, etc.). Activity recognition using smartphones is a classic multivariate time-series classification problem,
which makes use of sensor data and extracts discriminative features from them to recognize activities by a classifier [10]. As we know, time-series data have a strong one-dimensional structure, in which the variables temporally nearby are highly correlated [11]. Traditional methods usually consist of two parts:
feature extraction and classification. They rely on extracting complex hand-crafted features which require laborious human intervention and leads to the incapability of pedestrian activities identification.

One of the challenges of activity recognition is~\it{feature extraction}. The activity recognition performance depends highly on the feature representations of the sensor data [10]. Recently, the concept of deep learning has attracted considerable attention. There are numerous applications based on deep learning, such as image processing [12], speech enhancement [13], intelligent transportation system [14], indoor localization [15], and so on. Many studies have confirmed that a deep learning model has a better feature representation capability and, accordingly, could more effectively deal with complexity classification tasks [16]. This is because the deep learning methods
fusing feature extraction and classification together with a neural network which can automatically learn proper features.

In this paper, we propose a deep learning-based method for indoor activity recognition by using the combination of data from multiple smartphone built-in sensors. A new convolutional neural network (CNN) has been designed for the one-dimensional sensor data to learn the proper features
automatically. Experiments show that the proposed method achieves approximately 98.33\% accuracy in identifying nine types of activities, including still, walk, upstairs, up elevator, up escalator, down
elevator, down escalator, downstairs and turning. The contribution of this paper is designing a deep learning framework to efficiently recognize activities, which can be used for indoor localization.


